A Compiler Assisted Scheduler for Detecting and Mitigating Cache-Based Side Channel Attacks

Side channel attacks steal secret keys by cleverly leveraging information leakages and can, therefore, break encryption. Thus, detection and mitigation of side channel attacks is a very important problem, but the solutions proposed in the literature have limitations in that they do not work in a real-world multi-tenancy setting on servers, have high false positives, or have high overheads. In this work, we demonstrate a compiler guided scheduler, Biscuit, that detects cache-based side channel attacks for processes scheduled on multi-tenancy server farms. A key element of this solution involves the use of a cache-miss model which is inserted by the compiler at the entrances of loop nests to predict the cache misses of the corresponding loop. Such inserted library calls, or beacons, convey the cache miss information to the scheduler at run time, which uses it to co-schedule processes such that their combined cache footprint does not exceed the maximum capacity of the last level cache. The scheduled processes are then monitored for actual vs predicted cache misses, and when an anomaly is detected, the scheduler performs a search to isolate the attacker. We show that Biscuit is able to detect and mitigate Prime+Probe, Flush+Reload, and Flush+Flush attacks on OpenSSL cryptography algorithms with an F-score of 1, and also to detect and mitigate degradation of service on a vision application suite with an F-score of 0.9375. Under a no-attack scenario, the scheme poses low overheads (up to a maximum of 6 percent). In the case of an attack, the scheme ends up with less than 11 percent overhead and is able to reduce the degradation of service in some cases by 40 percent. With these many desirable features such as an ability to deal with multi-tenancy, its ability to detect attacks early, its ability to mitigate those attacks, and low runtime overheads, Biscuit is a practical solution.

==> texes/evaluationfigures.tex <==
\begin{figure*}[]
\centering
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/AES_Time.png}
 \caption{AES Time}%\label{fig:pLoop4}
\label{fig:AESTime}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/RSA_Time.png}
 \caption{RSA Time}%\label{fig:pLoop4}
\label{fig:RSATime}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/ECSDA_Time.png}
 \caption{ECSDA Time}%\label{fig:pLoop4}
\label{fig:ECSDATime}
\end{subfigure}
\caption{Timing between CFS and Biscuit for OpenSSL Algorithms alongside no attacks }
\label{fig:SSLTiming}
\end{figure*}


\begin{figure*}[]
\centering
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/Disparity_Time.png}
 \caption{Disparity Time}%\label{fig:pLoop4}
\label{fig:DisTime}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/Multi_Ncut.png}
 \caption{Multi-NCut Time}%\label{fig:pLoop4}
\label{fig:MCTime}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/SVM_Time.png}
 \caption{SVM Time}%\label{fig:pLoop4}
\label{fig:SVMTime}
\end{subfigure}

\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/Localization_Time.png}
 \caption{Localization Time}%\label{fig:pLoop4}
\label{fig:LocalTime}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/Mser_Time.png}
 \caption{Mser Time}%\label{fig:pLoop4}
\label{fig:MserTime}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/Sift_Time.png}
 \caption{Sift Time}%\label{fig:pLoop4}
\label{fig:SiftTime}
\end{subfigure}

\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/Stitch_Time.png}
 \caption{Stitch Time}%\label{fig:pLoop4}
\label{fig:StitchTime}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/Tex_Time.png}
 \caption{Texture Synthesis Time}%\label{fig:pLoop4}
\label{fig:TSTime}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/Tracking_Time.png}
 \caption{Tracking Time}%\label{fig:pLoop4}
\label{fig:TrackingTime}
\end{subfigure}
\caption{Timing between CFS and Biscuit for SDVBS Algorithms alongside no attacks }
\label{fig:SDVBSTiming}
\end{figure*}

\begin{figure*}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/AESFR.png}
 \caption{Flush+Reload Misses}%\label{fig:pLoop4}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/AESFF.png}
 \caption{Flush+Flush Misses}%\label{fig:pLoop4}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/AESPP.png}
 \caption{Prime+Probe Misses}%\label{fig:pLoop4}
\end{subfigure}
\caption{AES Misses}%\label{fig:pLoop4}
\label{fig:AESMiss}
\end{figure*}

\begin{figure*}[]
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/RSAFR.png}
 \caption{Flush+Reload Misses}%\label{fig:pLoop4}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/RSAFF.png}
 \caption{Flush+Flush Misses}%\label{fig:pLoop4}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/RSAPP.png}
 \caption{Prime+Probe Misses}%\label{fig:pLoop4}
\end{subfigure}
\caption{RSA Misses}%\label{fig:pLoop4}
\label{fig:RSAMISSES}
\end{figure*}

\begin{figure*}[]
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/ECSDAFR.png}
 \caption{Flush+Reload Misses}%\label{fig:pLoop4}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/ECSDAFF.png}
 \caption{Flush+Flush Misses}%\label{fig:pLoop4}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/ECSDAPP.png}
 \caption{Prime+Probe Misses}%\label{fig:pLoop4}
\end{subfigure}
\caption{ECDSA Misses}%\label{fig:pLoop4}
\label{fig:ECDSAMISSES}
\end{figure*}



\begin{figure*}[]
\centering
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/disparitymisses.png}
 \caption{Disparity Misses}%\label{fig:pLoop4}
\label{fig:DisMisses}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/SVMMISSES.png}
 \caption{SVM Misses}%\label{fig:pLoop4}
\label{fig:SVMMisses}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/MULTINCUTMISSES.png}
 \caption{Multi-NCut Misses}%\label{fig:pLoop4}
\label{fig:MCMisses}
\end{subfigure}

\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/LocalizationMisses.png}
 \caption{Localization Misses}%\label{fig:pLoop4}
\label{fig:LocalMisses}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/MSERMISSES.png}
 \caption{Mser Misses}%\label{fig:pLoop4}
\label{fig:MserMisses}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/SIFTMISSES.png}
 \caption{Sift Misses}%\label{fig:pLoop4}
\label{fig:SiftMisses}
\end{subfigure}

\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/STITCHMISSES.png}
 \caption{Stitch Misses}%\label{fig:pLoop4}
\label{fig:StitchMisses}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/TSMISSES.png}
 \caption{Texture Synthesis Misses}%\label{fig:pLoop4}
\label{fig:TSMisses}
\end{subfigure}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=2.2in]{figures/TRACKINGMISSES.png}
 \caption{Tracking Misses}%\label{fig:pLoop4}
\label{fig:TrackingMisses}
\end{subfigure}
\caption{SDVBS Cache Misses}
\label{fig:SDVBSMISSES}
\end{figure*}

==> texes/missesfigures.tex <==
\begin{figure*}
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/RSAFR.png}
 \caption{Flush+Reload Misses}%\label{fig:pLoop4}
\end{subfigure}\hfill
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/RSAFF.png}
 \caption{Flush+Flush Misses}%\label{fig:pLoop4}
\end{subfigure}\hfill
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/RSAPP.png}
 \caption{Prime+Probe Misses}%\label{fig:pLoop4}
\end{subfigure}\hfill
\caption{RSA Misses}%\label{fig:pLoop4}
\label{fig:RSAMISSES}
\end{figure*}

\begin{figure*}
\centering
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/disparitymisses.png}
 \caption{Disparity Misses}%\label{fig:pLoop4}
\label{fig:DisMisses}
\end{subfigure}\hfill
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/SVMMISSES.png}
 \caption{SVM Misses}%\label{fig:pLoop4}
\label{fig:SVMMisses}
\end{subfigure}\hfill
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/MULTINCUTMISSES.png}
 \caption{Multi-NCut Misses}%\label{fig:pLoop4}
\label{fig:MCMisses}
\end{subfigure}\hfill
\caption{SDVBS Cache Misses}
\label{fig:SDVBSMISSES}
\end{figure*}

==> texes/timefigures.tex <==

\begin{figure*}[b]
\centering
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/AES_Time.png}
 \caption{AES Time}%\label{fig:pLoop4}
\label{fig:AESTime}
\end{subfigure}\hfill
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/RSA_Time.png}
 \caption{RSA Time}%\label{fig:pLoop4}
\label{fig:RSATime}
\end{subfigure}\hfill
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/ECSDA_Time.png}
 \caption{ECSDA Time}%\label{fig:pLoop4}
\label{fig:ECSDATime}
\end{subfigure}\hfill
\caption{Timing between CFS and Biscuit for OpenSSL Algorithms alongside no attacks }
\label{fig:SSLTiming}
\end{figure*}


\begin{figure*}[]
\centering
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/Disparity_Time.png}
 \caption{Disparity Time}%\label{fig:pLoop4}
\label{fig:DisTime}
\end{subfigure}\hfill
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/Multi_Ncut.png}
 \caption{Multi-NCut Time}%\label{fig:pLoop4}
\label{fig:MCTime}
\end{subfigure}\hfill
\begin{subfigure}{0.32\textwidth}
\centering\includegraphics[width=\textwidth]{figures/SVM_Time.png}
 \caption{SVM Time}%\label{fig:pLoop4}
\label{fig:SVMTime}
\end{subfigure}\hfill

\caption{Timing between CFS and Biscuit for SDVBS Algorithms alongside no attacks }
\label{fig:SDVBSTiming}
\end{figure*}
